Making Pre-trained Language Models Better Few-shot Learners

The recent GPT-3 model (Brown et al., 2020) achieves remarkable few-shot performance solely by leveraging a natural-language prompt and a few task demonstrations as input context. Inspired by their findings, we study few-shot learning in a more practical scenario, where we use smaller language models for which fine-tuning is computationally efficient. We present LM-BFF--better few-shot fine-tuning of language models--a suite of simple and complementary techniques for fine-tuning language models on a small number of annotated examples. Our approach includes (1) prompt-based fine-tuning together with a novel pipeline for automating prompt generation; and (2) a refined strategy for dynamically and selectively incorporating demonstrations into each context. Finally, we present a systematic evaluation for analyzing few-shot performance on a range of NLP tasks, including classification and regression. Our experiments demonstrate that our methods combine to dramatically outperform standard fine-tuning procedures in this low resource setting, achieving up to 30% absolute improvement, and 11% on average across all tasks. Our approach makes minimal assumptions on task resources and domain expertise, and hence constitutes a strong task-agnostic method for few-shot learning.

==> sections/analysis.tex <==
%!TEX root = ../main.tex

\section{Analysis}
\label{sec:analysis}


\subsection{Generated vs. manual prompts}

% \danqi{
%     Basically a large table showing that generated prompts are reasonable and provide enough diversity. It also removes human labor.
% }

\danqi{I am also thinking we need to discuss the imbalanced-class issue for SNLI tasks (zero-shot and after fine-tuning). }


% \danqi{I am thinking of picking one dataset from single-sentence tasks (SST-2?) and one dataset from sentence-pair tasks and show that
% \begin{itemize}
%     \item
%         Even with the fixed manual prompt, the choice of label words matter a lot. I would love to have the experiments we had before: 1) swapping negative and positive words; 2) randomly sample two words as label words.
%     \item
%         Fixing a set of label words, the choice of prompts matter a lot in terms of the final performance.
% \end{itemize}
% A figure is better. Maybe we will draw the conclusion the manually picked template is actually way better than the average ones and it is a tough-to-beat baseline.
% }


\input{tables/auto_search_compare.tex}

\input{tables/generated_template.tex}

In this section, we study the quality of our automatically generated prompts. This includes two parts: automatically generated templates (auto T) using manual label words and generated label words (auto L) using manual templates. Table~\ref{tab:auto_search} shows the results of using manual or automatic prompts on selected datasets. In most cases, auto T achieves comparable or even higher performance than manual prompts. Auto L can outperform manual prompts on some datasets, but there are also cases where auto L perform significantly worse than the original results.

To further analyze the automatic search results, we demonstrate some of the generated examples in Table~\ref{tab:generated_template}.
Generated templates fit the context and the manual label words for most cases.
For automatically generated label words, things are mixed: while most of them look intuitively reasonable, there are some abnormal label words (e.g., ``better'' for the negative class in SST-5). We believe this is due to the overfitting issue of automatic label word search.

% \subsection{Analysis of automatic search}


\subsection{Analysis of in-context learning}
\label{sec:in_context_analysis}

% \danqi{
%     Ablation studies on 1) better ways of sampling examples; 2) how many examples to pack into context.
% }

In this section we compare different variants of in-context fine-tuning. Table~\ref{tab:pair_ablation} reports the performance of in-context fine-tuning without filtering, filtered by RoBERTa and filtered by Sentence-BERT. Since RoBERTa does not provide sentence embedding directly, we use the mean pooling over representations at all positions.

From Table~\ref{tab:pair_ablation}, we can see that all variants outperform prompt-based fine-tuning on most tasks. Compared to the vanilla in-context fine-tuning, using either of the encoders leads to further boost.
Among them, Sentence-BERT filtering achieves the best performance, and we take it as the default in-context fine-tuning model. We acknowledge that Sentence-BERT is trained on SNLI~\cite{bowman2015large_snli}, MNLI~\cite{williams2018broad_mnli} and STS-B~\cite{cer2017semeval_sts-b} datasets, and this may contribute to the good performance in filtering.

\input{tables/pair_ablation}


%\subsection{Ensemble}

\subsection{Comparisons of pre-trained LMs}

\label{sec:analysis_bert}

% \danqi{I wonder if it is interesting to discuss BERT vs RoBERTa and segment embeddings at least. I remember we have some insightful findings there.}

\input{tables/bert.tex}

Table~\ref{tab:bert} shows the results of using BERT-large (uncased) and RoBERTa-large in our settings. Our in-context fine-tuning also works for BERT on some datasets, but the results are mixed compared to RoBERTa. This might be due to that BERT uses different segment embeddings to distinguish different parts of inputs (e.g., premise and hypothesis in NLI). There are only 2 pre-trained segment embeddings, and for in-context learning, we need to train new segment embeddings from scratch, which increases the instability of few-shot fine-tuning. 

%\subsection{Overfitting?}


\subsection{Sample Efficiency}


\begin{figure}
    \centering
    \includegraphics[width=0.235\textwidth]{figures/sample_sst2.pdf}
    \includegraphics[width=0.235\textwidth]{figures/sample_snli.pdf}
    \caption{Performance of fine-tuning and our LM-BFF with different $K$ (numbers of instances per class).
    \todo{The last point of SNLI is a placeholder.}}
    \label{fig:sample}
\end{figure}  

It is interesting to see how the standard fine-tuning and our method (LM-BFF) perform with increasing K and where we stand compared to taking the full dataset fine-tuning. Figure~\ref{fig:sample} gives a comparison on SST-2 and SNLI. 
We can see that for simple tasks like SST-2 (also see MR, CR and MPQA in Table~\ref{tab:main_results}), LM-BFF already achieves comparable results to full dataset fine-tuning only with 32 examples. 
With increasing $K$, LM-BFF continues to show performance gain compared to standard fine-tuning, until after $K=256$ where the two approaches converge.


==> tables/compare_related_work.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
\begin{center}
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Prompt} & \multirow{2}{*}{In-context} & \multirow{2}{*}{Fine-tune}  & Super & Semi- \\
&  &  &  & large & supervised \\
\midrule
GPT-3 & \cmark & \cmark & \xmark & Yes & No \\
PET & \cmark & \xmark & \cmark & No & Yes \\
Ours  & \cmark & \cmark & \cmark & No & No  \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Compare \tianyu{Do we want to have a table like this to make the difference clearer?}}
\label{tab:compare_related_work}
\end{table}


==> tables/t5_search.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \begin{center}
    \centering
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{lc}
        \toprule
        % \multicolumn{2}{c}{single-sentence} \\
        % \midrule
        \multirow{2}{*}{$\xinput=$\{\sent\} }& \maskx~$\lwordmap(y)$~\masky~\sent\\
         & \sent~\maskx~$\lwordmap(y)$~\masky\\
        % \midrule
        % \multicolumn{2}{c}{sentence-pair} \\
         \midrule
        $\xinput=$\{\firstsent,\secondsent\} & \firstsent~\maskx~$\lwordmap(y)$~\masky~\secondsent\\
        \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{Input format $\template_{\mathrm{gen}}(\xinput, y)$ for T5 automatic generation of templates. \maskx and \masky are mask tokens in T5. $y$ and $\lwordmap(y)$ are the class of the example and its corresponding label word. \todo{This table doesn't add much. Let's move it to the text.}}
    \label{tab:t5_template}
\end{table}

